Recovery Guarantee of Non-negative Matrix Factorization via Alternating Updates

Non-negative matrix factorization is a popular tool for decomposing data into feature and weight matrices under non-negativity constraints. It enjoys practical success but is poorly understood theoretically. This paper proposes an algorithm that alternates between decoding the weights and updating the features, and shows that assuming a generative model of the data, it provably recovers the ground-truth under fairly mild conditions. In particular, its only essential requirement on features is linear independence. Furthermore, the algorithm uses ReLU to exploit the non-negativity for decoding the weights, and thus can tolerate adversarial noise that can potentially be as large as the signal, and can tolerate unbiased noise much larger than the signal. The analysis relies on a carefully designed coupling between two potential functions, which we believe is of independent interest.

==> algo_purification_old.tex <==
\section{Main algorithm and results} \label{sec:algo_purification}

\begin{algorithm}[!th]
\caption{Main algorithm: Purification}\label{alg:main_sim_noise}
\begin{algorithmic}[1]
\REQUIRE{initialization $\bA^{(0)}$, threshold $\alpha$, step size $\eta$, scaling factor $\etaratio$, sample size $N$, iterations $T$}
\FOR{$t = 0, 1, 2, ..., T - 1$}
\STATE Draw examples $y_1, \dots, y_N$.
\STATE (Decode)  Solve the following convex program for $\bA^{\dagger} $: \\
 $
	 \qquad\qquad\qquad\qquad
	 \min \|\bA^{\dagger}\|_{\infty} \text{ s.t. }\bA^{\dagger}  \rbr{\bA^{(t)}} = \bI 
	$
\\
\qquad\qquad Set $x = \phi_{\alpha} (\bA^{\dagger} y)$ for each example $y$. \hfill \textit{// See main text for the definition of $\phi_\alpha$}
\STATE (Encode)
Update the feature matrix \\
$
  \qquad\qquad \qquad\qquad 
	\bA^{(t + 1)} = \left(1 - \eta \right)\bA^{(t)} + \etaratio \eta \hat{\E}\left[ (y - y')(x - x')^{\top}\right]
$\\
where $\hat{\E}$ is over independent uniform $y, y'$ from $\cbr{y_1, \dots, y_N}$,  and $x, x'$ are their decodings.  
\ENDFOR
\ENSURE{$\bA$ where $\bA_i  = {\bA^{(T)}_i } \big / \| \bA^{(T)}_i \|_1$}
\end{algorithmic}
\end{algorithm}

Our main algorithm is presented in Algorithm~\ref{alg:main_sim_noise}.  
It keeps a working feature matrix and operates in iterations. In each iteration, it first compute the weights for $N$ examples (decoding), and then use the computed weights to update the feature matrix (encoding). 

The decoding is simply multiplying the example by the pseudo-inverse of the current feature matrix and then passing it through a threshold function $\phi_\alpha$.  The pseudo-inverse with minimum infinity norm is used so as to maximize the robustness to noise (see the theorems). The threshold function operates element-wisely on the input vector $v$, and for an element $v_i$, it is defined as
\Anote{Again, we need a new name for this.. }
\begin{align}
   \phi_\alpha(v_i) & = \max\cbr{v_i - \alpha, 0}.
\end{align}
To get some sense about the decoding, suppose the current feature matrix is the ground-truth. Then 
$
  \bA^{\dagger} y = \bA^{\dagger} \bAg x^* + \bA^{\dagger} \noise = x^* + \bA^{\dagger} \noise.
$
So we would like to use a small $\bA^{\dagger}$ and use threshold to remove the noise term.

In the encoding step, the algorithm move the feature matrix along the direction $\E\left[ (y - y')(x - x')^{\top}\right]$. Suppose we have independent $x^*_i$'s, perfect decoding and no noise, then $\E\left[ (y - y')(x - x')^{\top}\right] = \bA^*$, and thus it is moving towards the ground-truth.  
Without those ideal conditions, we need to choose a proper step size, which is tune by the parameters $\eta$ and $r$. 

At the end, the algorithm simply outputs the scaled features with unit norm.  The output enjoys the following guarantee in the adversarial noise model.

We let $(\bAg)^\dagger$ denote the matrix satisfying $(\bAg)^\dagger \bAg = \bI$; if there are multiple such matrices we let it denote the one with minimum $\|(\bAg)^\dagger\|_\infty$.

\begin{thm}[Adversarial noise] \label{thm:main_correlated_noise}
There exists a \emph{absolute constant} $\abscc$ such that when Assumption (\textbf{A0})-(\textbf{A3}) and (\textbf{N1}) are satisfied with $l = 0.1$, $\xsu \le 2 \xsl$, $\xexpc^3 \le \abscc \xsl^2 n$, $\cnoise   \le \frac{ \abscc c}{\max\cbr{\mu^2 \nword,  \mu^4 \ntopic  \nbr{ \rbr{\bAg}^\dagger}_\infty} }$  for $0 \le c\le 1$, $ \mu = \xexpc/\xsl$,  and $\nbr{\titime{\bN}{0}}_{1} \le \frac{c}{10}$, $\nbr{\titime{\bN}{0}}_{\infty} \le \frac{1}{ 8 \nbr{(\bAg)^\dagger}_\infty}$, then there exist $\alpha, \eta, r$ such that for every $\epsilon$ and  $N  = \mathrm{poly}(\ntopic, \nword, 1/\epsilon)$ the following holds: After $T = O\rbr{ \ln \frac{1}{\epsilon}}$ iterations, Algorithm~\ref{alg:main_sim_noise} outputs a solution $\bA$ satisfying that for any $i \in [\ntopic]$, 
 $\nbr{\bA_i - \bAg_i}_1 \le \epsilon + c$.
%$\bA = \bAg \rbr{\widehat{\bSigma} + \widehat{\bE} } + \widehat{\bN}$, where $\widehat{\bSigma}$ is diagonal and $\widehat{\bE}$ is off-diagonal, satisfying
%$$
%\rbr{1 - \epsilon - c} \bI \preceq \widehat{\bSigma} \preceq  \rbr{1 + \epsilon + c}  \bI,  ~~\sym{\widehat{\bE} } \le \epsilon + c, ~~\sym{\widehat{\bN} } = c.
%$$
 \end{thm}

\paragraph{Remarks} 
Under mild conditions and with proper parameters, our algorithm recovers the ground-truth in a geometric rate. It can achieve arbitrary small recovery error in the noiseless setting, and achieve error up to the noise limit even with adversarial noise whose level is comparable to the signal.

The conditions on $\xexpc, \xsl, \xsu$ roughly mean that each feature needs to appear with reasonable probability. $\xsu \le 2\xsl$ means that their proportions are quite even. This may be a mild restriction for some applications, so we propose a pre-processing step that can relax this in the next section.  

The condition on $\ell$ means that a constant warm start is sufficient for our algorithm to converge, which is much better than previous work such as~\cite{AwaRis15}. Indeed, in that work, the $\ell$ needs to even depend on the dynamic range of the entries of $\bA^*$ which is problematic in practice. 

The conditions allow a rather general family of distributions, so we point out an important special case to provide a more concrete sense of the parameters. 
A natural distribution that satisfies the conditions is the uniform $s$-sparse distribution, where independently $x^*_i = 1$ with probability $\frac{s}{\ntopic}$ and $0$ otherwise. Then $C_1 = c_2 = C_2 = s$, and $\mu = 1$. Our algorithm just requires $s \le \abscc n$ for a fixed constant $\abscc$. So it works for uniform sparse distributions even when the sparsity is linear, which is an order of magnitude larger than in the dictionary learning regime. Moreover, we have no structural assumptions on $\bAg$. 

Continuing the above example for the noise parameters:
with adversarial noise, it can still recover the features up to the noise limit: the error $\nbr{\bA - \bAg}_1$ is $O(c)$, even when each data point has adversarial noise with $\ell_1$ norm as large as  $\| \nu \|_1 = \cnoise \nword = \Omega(c)$ when $m \ge n \|\rbr{\bAg}^\dagger\|_\infty$.
\Anote{I don't like the next sentence. I don't know why ``in most cases we are interested in'' the $\infty$-condition number is small. 
Maybe just give for the time being an example of a good case -- which is $e_i$ for each column i, and a bad case -- columns are all nearly the same. } In most cases we are interested in,  $\|\rbr{\bAg}^\dagger\|_\infty$ is small; in the extreme case where the columns of $\bAg$ are basis vectors, $\|\rbr{\bAg}^\dagger\|_\infty = 1$. 
In such cases, the recovery error is in the same order as the adversarial noise level in each data point. Furthermore, $s$ can be as small as a constant, then $\|\bAg x^*\|_1 = O(1)$, the same order as the noise.  Our algorithm still works in this regime.

A similar theorem holds for the unbiased noise model.
\begin{thm}[Unbiased noise] \label{thm:main_unbiased_noise}
Suppose Assumption (\textbf{A0})-(\textbf{A3}) and (\textbf{N2}) are satisfied with $\cnoise =  \frac{\mathcal{G} c\sqrt{\ntopic}}{\max\cbr{ \mu \nword, \mu\ntopic \nbr{\rbr{\bAg}^\dagger}_\infty }  }$ and the other parameters set as in Theorem~\ref{thm:main_correlated_noise}. Then the same guarantee in Theorem~\ref{thm:main_correlated_noise} holds.
 \end{thm}

\textbf{Remarks}
With unbiased noise which is commonly assumed in many applications, the algorithm can tolerate noise level $\sqrt{n}$ larger than the adversarial case. This means that $\| \bAg - \bA \|_1$ is in the order of $O\rbr{\| \nu \|_1 / \sqrt{n} } $, 
even smaller than the noise in each data point. 
The noise $\| \nu \|_1$ can be as larger as $O(\sqrt{n})$, which is much larger than the signal when the signal is constant (recall the example above). 
This is a bit counter-intuitive, but is possible since we exploit the average of the noise for cancellation, and also use thresholding to remove noise spread out in the coordinates.

\Anote{Why is this here? I think we should move this to the conclusion maybe?}
\textbf{Future directions} Our algorithm, at least theoretically, can only be applied to the case when each coordinate of $x^*$ are un-correlated (Assumption (\textbf{A2})). Indeed, since NMF is known to be NP-hard in the worst case and we essentially have no assumption on $\bAg$, we need to have some assumption on the distribution of $x^*$. An interesting future direction is to extend our algorithm to the case where the coordinates of $x^*$ are correlated. 
%\Anote{This seems unnecessary to me. This is not an unstandard assumption in dict. learning and similar settings. If anything, the drawback is the warm start which is not algorithmic} 
%\yingyu{IMO the discussion about the drawback can be moved to the discussion after the results or the conclusion as future work. }

\subsection{Analysis: intuition}

A natural approach typically employed to analyze algorithms for non-convex problems is to define a function on the intermediate solution $\bA$ and the ground-truth $\bAg$ measuring their distance and then show that the function decreases at each step. However, a single potential function is not enough in our case, and we introduce a new framework to measure the progress by denoting the intermediate solution and the update as (omit the superscript $(t)$)
$$ \bA  = \bAg (\bSigma + \bE) + \bN, \label{eqn:intuition:update01} 
\quad  \hat{\E}[(y - y')(x - x')^{\top}]  = \bAg(\btSigma + \btE) + \btN,  \label{eqn:intuition:update02}
$$
where $\bSigma, \btSigma$ are diagonal, $\bE, \btE$ are off-diagonal, and $\bN, \btN$ are the terms caused by the noise and may lie outside the span of $\bAg$. To illustrate the intuition, we focus on the noiseless case. Since $\bA_i = \bSigma_{i,i} \bAg_i + \sum_{j \neq i}\bE_{j,i} \bAg_j$,  if the ratio between $\nbr{\bE_i}  = \sum_{j \neq i} \abr{\bE_{j,i}}$  and  $\bSigma_{i,i}$ gets smaller, then the algorithm is making progress; if the ratio is large at the end, a normalization of $\bA_i$ gives a good approximation of $\bAg_i$.\footnote{It is tempting to do the normalization at each iteration and use $\max_{i} \nbr{ \bA_i - \bAg_i}$ as the Lyapunov function. However, $\bE_{j,i}$ can be negative and normalization at each iteration can blow up $\bE_{j,i}$, then the algorithm may fail.} 

So it suffices to show that $\bSigma_{i,i}$ is always about a constant while $\nbr{\bE_i}$ decreases at each iteration. To see how to achieve this, we now turn to the update rule in the algorithm. 
Again for demonstrating idea, we pretend that we have infinite data.  Then after some calculation, we have
\begin{align} 
  & \bSigma_{i,i} \leftarrow (1- \eta)  \bSigma_{i,i} +  r \eta \btSigma_{i,i}, &  \btSigma_{i,i} =  \E \sbr{ \rbr{x^*_i - (x')^*_i} \rbr{x_i - x'_i}^{\top}},  \label{eqn:intuition:update1} \\
  & \bE_{j,i}   \leftarrow (1- \eta)  \bE_{j,i} +  r \eta \btE_{j,i}, & \btE_{j,i}  = \E \sbr{ \rbr{x^*_j - (x')^*_j} \rbr{x_i - x'_i}^{\top}}, \label{eqn:intuition:update2}
\end{align}
where $x, x'$ are the decoding for $x^*, (x')^*$ respectively:
\begin{align} \label{eqn:intuition:decode}
  & x = \phi_\alpha\rbr{ (\bSigma + \bE)^{-1} x^* }, 
	& x' = \phi_\alpha\rbr{ (\bSigma + \bE)^{-1} (x')^* }.
\end{align}

Now we consider the decoding to see why the thresholding is important. If $\bE = 0$ and $\bSigma$ is roughly a scaled identity, then $x$ is just a scaled $x^*$, resulting in a large $\btSigma_{i,i}$ and small $\btE_{j,i}$'s. In the presence of $\bE$, ignoring the higher order terms, 
\begin{align} \label{eqn:intuition:inverse}
  (\bSigma + \bE)^{-1}  & \approx \bSigma^{-1} - \bSigma^{-1}\bE\bSigma^{-1}
\end{align}
Then without thresholding, we still have larger positive signals on a few coordinates of $x$ where $x^*_i$ is large, but due to $\bSigma^{-1}\bE\bSigma^{-1}$, we also have errors on most of the coordinates in $x$. These errors when summed up will be comparable or even larger than the signals, and the algorithm will fail. However, since the signals are non-negative and most coordinates with errors only have small values,  thresholding properly can remove those errors while keeping a large fraction of the signals. This leads to large $\btSigma_{i,i}$ and small $\btE_{j,i}$'s, and then we can choose an $r$ such that $\bE_{j,i}$'s keep decreasing while $\bSigma_{i,i}$'s stay in a certain range. 

To get a quantitative bound, we divide $\bE$ into its positive part $\bE_+$ and its negative part $\bE_-$:
\begin{align}
 & \sbr{\bE_+}_{i,j} = \max\cbr{\bE_{i,j}, 0}, 
& \sbr{\bE_-}_{i,j} = \max\cbr{-\bE_{i,j}, 0}.
\end{align}
The reason to do so is quite subtle. Roughly speaking, by \eqnref{eqn:intuition:update2}\eqnref{eqn:intuition:decode}\eqnref{eqn:intuition:inverse},  $-\bE_{i,j}$ affects $\btE_{j,i}$ (not  $\btE_{i,j}$ due to the transpose in the update rule), which then updates $\bE_{j,i}$. 
More precisely, when $\bE_{i,j}$ is negative, $\sbr{(\bSigma + \bE)^{-1}x^*}_i$ will tend to be more positive and can go pass the threshold. Therefore, $\bE_{j, i}$ will turn to be more positive at next iteration. On the other hand, when $\bE_{i,j}$ is positive, $\sbr{(\bSigma + \bE)^{-1}x^*}_i$ will tend to be more negative and flattened to zero by the threshold function. Therefore, $\bE_{j, i}$ will \emph{not} be more negative at next iteration. Intuitively, we will have for positive and negative parts of $\bE$:
$$
\text{postive}^{(t + 1)} \leftarrow (1 - \eta) \text{positive}^{(t)} + (\eta) \text{negative}^{(t)}, \quad \text{negative}^{(t + 1)} \leftarrow (1 - \eta) \text{negative}^{(t)} + (\varepsilon \eta) \text{positive}^{(t)}
$$
for a small $\varepsilon \ll 1$. Due to the small $\epsilon$, we couple the two parts and conclude that a weighted average of them will decrease, which implies that $\|\bE\|_s$ is small at the end.
 

==> discussion.tex <==
\section{Discussion} \label{sec:discussion}

noise in the equilibration

relaxing conditional independence; connection to topic model

potential connections of the threshold function to neural plausible updates





==> purification_proof_sketch_old.tex <==

\subsection{Analysis: proof sketch}

Here we describe a proof sketch while the complete proof is presented in the appendix.

\textbf{One iteration}
We focus on one update and omit the superscript $(t)$. 
Recall the definitions of $\bE$, $\bSigma$ and $\bN$ in \eqnref{eqn:intuition:update01}, and $\btE$, $\btSigma$ and $\btN$ in \eqnref{eqn:intuition:update02}. Our goal is to derive lower and upper bounds for $\btE$, $\btSigma$ and $\btN$, assuming that $\bSigma_{i,i}$ falls into some constant range around 1, while $\bE$ and $\bN$ are small. 
This will allow doing induction on them.

First, begin with the decoding. Some calculation shows that, the decoding for $y = \bA^* x^* + \noise$ is
\begin{align}
x & = \phi_{\alpha}\rbr{ \forder x^* + \xi }.
\end{align}
where we use the notations
\begin{align}
  \forder  = \left( \bSigma + \bE \right)^{-1}, ~~
	\xi = - \bA^\dagger \bN \forder x^* +  \bA^\dagger \noise.
\end{align}

Now, we can present our key lemma bounding $\btE$. 
\begin{lem}[Main: Bound on $\btE$] \label{lem:update_E}
Suppose $\nbr{\xi}_{\infty} \le \nthres < \alpha$ almost surely. 
For all $i, j \in [\ntopic]$, $i \not= j$, \\
(1) if $\forder_{i, j} < 0$, then 
$
  \left| \btE_{j, i} \right|  \le  \frac{4 \xexpc^2  \| \forder^i \|_1
}{\ntopic^2 (\alpha - \nthres)}  \rbr{ \left| \forder_{i, j} \right| + \nthres},
$
\\
(2) if $\forder_{i, j} \ge 0$, then \\
$~~~~~~~~
- B - \frac{2 \xexpc^2}{\ntopic^2} \forder_{i, j}
\le
  \abr{\btE_{j, i} } 
	\le 
	B + 2 \E[(x_j^*)^2] \forder_{i, j}, \textnormal{where}~ B=\frac{8\xexpc \nthres}{\ntopic (\alpha - \nthres)} \rbr{ \frac{\xexpc \| \forder^i \|_1 }{n} + \forder_{i, j}}.
$
\end{lem}

To parse the lemma, we first simplify some variables in it. With the assumptions on $\bSigma,\bE,$ and $\bN$, we can show that $\nthres = O(1)$, $\| \forder^i \|_1 = O(1)$. 
So the bound for $\forder_{i, j}<0$ is simplified to 
$ 
  \left| \btE_{j, i} \right|  \le O\rbr{ \frac{1}{n^2} \bE_{i,j} },
$
a very small value. Then the update $\bE \leftarrow (1-\eta) \bE + r\eta \btE$ decreases $|\bE_{j, i}|$.
This matches what is described in the intuition: $\forder \approx \bSigma^{-1} - \bSigma^{-1}\bE\bSigma^{-1}$, so $\forder_{i, j}<0$ corresponds roughly to $\bE_{i,j} > 0$, in which case  $|\bE_{j, i}|$ decreases.

What is most interesting is the case when $\forder_{i, j}\ge 0$ (roughly $\bE_{i,j} < 0$). In this case, the bound simplifies to 
$
   - O(1/n^2)  \le \btE_{j, i} \le O\rbr{ 1/n^2 } + 2\xsu\forder_{i,j}/\ntopic.
$
The upper bound is much larger, corresponding to the intuition that  negative $\bE_{i,j} $ can contribute a large positive value to $\bE_{j,i}$.  Fortunately, all the other bounds are much smaller, which allows us to show that a  Lyapunov function that couples Case (1) and Case (2) in Lemma~\ref{lem:update_E} actually decreases; see the induction below.

Finally, we also have the following bounds for $\btSigma$ and $\btN$. 
\begin{lem}[Main: Bound on $\btSigma$] \label{lem:update_diag}
Suppose $\nbr{\xi}_\infty \le \nthres < \alpha$ almost surely, and $\bSigma \succeq \frac{1}{2} \bI$. Let $\gorder = \forder - \bSigma^{-1}$. 
Then for any $i \in [\ntopic]$,  \\
$~~~~~~~~
\btSigma_{i, i } \ge 
\E\sbr{\rbr{x_i^*}^2} \rbr{ 2 \bSigma^{-1}_{i, i} - 2 \abr{\gorder_{i,i} } } - \frac{2\xexpc}{\ntopic} \rbr{  \alpha +2\nthres  + \frac{\xexpc}{\ntopic} \bSigma^{-1}_{i, i} + \frac{2\xexpc}{\ntopic}  \nbr{ \sbr{ \gorder}^i  }_1   },
\\
~~~~~~~~
  \btSigma_{i, i } \le  
\E\sbr{\rbr{x_i^*}^2} \rbr{ 2 \bSigma^{-1}_{i, i} + 2 \abr{\gorder_{i,i} } } + \frac{2\xexpc}{\ntopic} \rbr{   \nthres  + \frac{\xexpc}{\ntopic}  \nbr{ \sbr{ \gorder}^i  }_1   }.
$
\end{lem}

\begin{lem}[Main: Bound on $\btN$] \label{lem:bound_error}
Suppose $\nbr{\xi}_\infty \le \nthres < \alpha$ almost surely, $\sym{\bE} \le \ell$,  and $ \bSigma \succeq (1-\ell)\bI$. 
Let $
 \bNs  = \hat{\E}[(y - y')(x - x')^{\top}]  - \E[(y - y')(x - x')^{\top}].
$
For any $i \in [m], j \in [n]$,

(1) if the noise is adversarial (Assumption (\textbf{N1})), then 
$
\abr{ \btN_{i,j} }\le \frac{4 \cnoise \xexpc }{(1 - 2 \ell)^2 n  (\alpha - \rho)} + \abr{ [\bN_s]_{i,j}},
$

(2) if the noise is unbiased (Assumption (\textbf{N2})) and $\|\bA^{\dagger} \nu \|_{\infty} \le \rho' < \alpha$, then \\
$~~~~~~~~
  \abr{\btN_{i,j} } \le   \frac{2 \xexpc \cnoise \rho' (1 + \| \bA^{\dagger} \bN \|_{\infty})}{(1 - 2 \ell)  n (\alpha - \rho')}  + \abr{ \sbr{\bN_s}_{i,j} }.
$
\end{lem}

The bound on $\btSigma_{i,i}$ can be simplified to $2\btSigma_{i,i}^{-1} \E\sbr{(x_i^*)^2} \pm O(1/n)$. The bound for the adversarial noise is $O\rbr{\frac{\cnoise}{n} + \abr{ [\bN_s]_{i,j}} }$, and for the unbiased noise is $O\rbr{\frac{\cnoise \rho'}{n} + \abr{ [\bN_s]_{i,j}} }$. The extra $\rho'$ is important, since it is in the order of $1/n$ and leads to better tolerance to noise.

\textbf{Induction by iterations}
We now show how to use the three lemmas to prove the theorem for the adversarial noise, and that for the unbiased noise is similar. 

Let $a_t := \sym{ \pt{\bE} } $ and $b_t := \sym{ \nt{\bE} } $, and choose $\eta = \ell/6$.
We begin with proving the following three claims by induction on $t$: at the beginning of iteration $t$, 
\begin{itemize}
\item[(1)] $(1 - \ell)\bI \preceq \titime{\bSigma}{t} $ 
\item[(2)]  $\sym{\titime{\bE}{t}} \le  1/8$, and if $t > 0$, then
$
  a_{t} + \beta b_{t} \le  \rbr{1-\frac{1}{25}\eta }  \rbr{ a_{t-1} + \beta b_{t-1}} + \eta h,
$
for some $\beta \in (1, 8)$, and some small value $h$,
\item[(3)] $\sym{\titime{\bN}{t}} \le c/10$. %  \nbr{\titime{\bN}{t}}_\infty \le \frac{1}{8} \nbr{(\bAg)^\dagger}_\infty
\end{itemize}
The most interesting part is the second claim. At a high level, by Lemma~\ref{lem:update_E}, we can show that
\begin{align}
a_{t+1} &  \le  \rbr{1-\frac{3}{25}\eta  } a_{t}  +  7\eta b_t + \eta h, \label{eqn:at}
\\
b_{t+1} &  \le  \rbr{1- \frac{24}{25}\eta  } b_{t}  +  \frac{1}{100}\eta a_t + \eta h. \label{eqn:bt}
\end{align}
Notice that the contribution of $b_t$ to $a_{t+1}$ is quite large (due to the larger upper bound in Case (2) in Lemma~\ref{lem:update_E}), but the other terms are much nicer, such as the small contribution of $a_t$ to $b_{t+1}$.  This allows to choose a $\beta \in (1,8)$ so that \eqnref{eqn:at} plus $\beta$ times \eqnref{eqn:bt} leads to the desired recurrence in the second claim. In other words, $a_{t+1} + \beta b_{t+1}$ is our Lyapunov function which decreases at each iteration up to the level $h$.  The other claims can also be proved by the corresponding lemmas.
Then the theorem follows from the three claims. 


%Suppose $\bSigma = \bI$, then by \eqnref{eqn:intuition:update2}\eqnref{eqn:intuition:decode}\eqnref{eqn:intuition:inverse}, 
%\begin{align*}
 %\btE_{j,i}  & = 2\E \sbr{ x^*_j \rbr{x_i - x'_i}} \approx 
%2 \E \sbr{x^*_j \rbr{ \phi_\alpha \rbr{ x_i^* - \sum_{k=1}^m \bE_{i,k} x_k^*} -  \phi_\alpha\rbr{ (x_i')^* - \sum_{k=1}^m \bE_{i,k} (x_k')^*}  }  }.
%\end{align*}
%The terms $-\bE_{i,k} x_k^* (k\neq j)$ will be roughly canceled, but $-\bE_{i,j} x_j^*$ is coupled with the $x_j^*$ under the expectation and will stand out. 
%So $\bE_{i,j}$ affects $\btE_{j,i}$ and thus $\bE_{j,i}$ (notice the transpose in the update rule!) 
%More precisely, when $\bE_{i,j}$ is negative and $\bE_{j,i}$ is positive, $x_i - x'_i$ will tend to be more positive, which cannot be taken care of by the thresholding, and thus $\btE_{j,i}$ and $\bE_{j,i}$ will tend to be more positive. Then $\sym{\bE}$ can actually increase. 
